Task-Induced Representation Learning

In this work, we evaluate the effectiveness of representation learning approaches for decision making in visually complex environments. Representation learning is essential for effective reinforcement learning (RL) from high-dimensional inputs. Unsupervised representation learning approaches based on reconstruction, prediction or contrastive learning have shown substantial learning efficiency gains. Yet, they have mostly been evaluated in clean laboratory or simulated settings. In contrast, real environments are visually complex and contain substantial amounts of clutter and distractors. Unsupervised representations will learn to model such distractors, potentially impairing the agent's learning efficiency. In contrast, an alternative class of approaches, which we call task-induced representation learning, leverages task information such as rewards or demonstrations from prior tasks to focus on task-relevant parts of the scene and ignore distractors. We investigate the effectiveness of unsupervised and task-induced representation learning approaches on four visually complex environments, from Distracting DMControl to the CARLA driving simulator. For both, RL and imitation learning, we find that representation learning generally improves sample efficiency on unseen tasks even in visually complex scenes and that task-induced representations can double learning efficiency compared to unsupervised alternatives. Code is available at https://clvrai.com/tarp.

==> Task-Induced Representation Learning_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}t}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Task-Induced Representation Learning_arXiv/sections/abstract.tex <==
\begin{abstract}

In this work, we evaluate the effectiveness of representation learning approaches for decision making in visually complex environments. Representation learning is essential for effective reinforcement learning (RL) from high-dimensional inputs. Unsupervised representation learning approaches based on reconstruction, prediction or contrastive learning have shown substantial learning efficiency gains. Yet, they have mostly been evaluated in clean laboratory or simulated settings. In contrast, real environments are visually complex and contain substantial amounts of clutter and distractors. Unsupervised representations will learn to model such distractors, potentially impairing the agent's learning efficiency. In contrast, an alternative class of approaches, which we call \emph{task-induced representation learning}, leverages task information such as rewards or demonstrations from prior tasks to focus on task-relevant parts of the scene and ignore distractors.
We investigate the effectiveness of unsupervised and task-induced representation learning approaches on four visually complex environments, from Distracting DMControl to the CARLA driving simulator. For both, RL and imitation learning, we find that representation learning generally improves sample efficiency on unseen tasks even in visually complex scenes and that task-induced representations can double learning efficiency compared to unsupervised alternatives. \footnote{Project website: \href{https://clvrai.com/tarp}{\url{clvrai.com/tarp}}}







\end{abstract}


==> Task-Induced Representation Learning_arXiv/sections/acknowledgement.tex <==
\section{Acknowledgement}
We thank our colleagues from the CLVR lab at USC for the valuable discussions that considerably helped to shape this work.

==> Task-Induced Representation Learning_arXiv/sections/approach.tex <==

\section{Problem Formulation}
\label{sec:problem_formulation}

Our goal is to efficiently learn a policy $\pi$ that solves a target task $T_\text{target}$ in an MDP defined by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{T}, R, \rho, \gamma)$ of states, actions, transition probabilities, rewards, initial state distribution, and discount factor. The policy is trained to maximize the discounted return $\mathbb{E}_{a_t \sim \pi} \big[ \sum_{t=0}^{T-1} \gamma^t R(s_t, a_t) \big]$.

We do not assume access to the underlying state $s$ of the MDP, but instead our policy receives a high-dimensional observation $x \in \mathcal{X}$ in every step, e.g.,~an image observation. To improve training efficiency, we aim to learn an encoder $\phi(x)$ which maps the input observation to a low-dimensional \emph{state representation} that is input to the policy $\pi(\phi(x))$. To learn this representation, we assume access to a dataset of past interactions $\mathcal{D} = \{\mathcal{D}_1, \dots, \mathcal{D}_N\}$ collected across $T_{1:N} \in \mathcal{T}$ tasks, with per-task datasets $\mathcal{D}_i = \{x_t, a_t, (r_t), ...\}$ of state-action trajectories and optional reward annotation. The set of training tasks does not include the target task $T_\text{target} \notin T_{1:N}$. We assume that the training data contains task information for prior tasks, e.g.,~in the form of step-wise reward annotations $r_t$ or by consisting of task demonstrations. Such task information can often be available at no extra cost, \eg if the data was collected from prior training runs~\citep{fu2020d4rl,gulcehre2020rl} or human teleoperation~\citep{mandlekar2018roboturk,cabi2019}. %

We follow~\citet{stooke2020decoupling} and test all representation learning approaches in two phases: we first train the representation encoder $\phi(x)$ from the offline dataset $\mathcal{D}$, then transfer its parameters to the policy $\pi(\phi(x))$ and optimize it on the downstream task, either freezing or finetuning the encoder parameters. This allows us to efficiently reuse data collected across prior tasks. %


    
    


\subsection{Unsupervised Representation Learning}
\label{sec:unsup_representation_learning}

Unsupervised representation learning approaches aim to learn the low-dimensional representation $\phi(x)$, by maximizing lower bounds on the mutual information $\max_\phi I\big(x, \phi(x)\big)$.

\paragraph{Generative Representation Learning.} Maximizes the mutual information via generative modeling, either of the current state (\textbf{reconstruction}) or of future states (\textbf{prediction}). A decoder $D(\phi(x))$ is trained by maximizing a lower bound on the data likelihood $p(x)$~\citep{kingma2014auto,rezende2014stochastic,denton2018stochastic,hafner2018learning}.

\paragraph{Contrastive Representation Learning.} Avoids training complex generative models by using contrastive objectives for maximizing the mutual information~\citep{oord2018representation,laskin2020curl,stooke2020decoupling}. During training, mini-batches of positive and negative data pairs are assembled, where positive pairs can for example constitute consecutive frames of the same trajectory while negative pairs mix frames across trajectories. The representation is then trained with the InfoNCE objective~\citep{gutmann2010noise,oord2018representation}, which is a lower bound on $I\big(x, \phi(x)\big)$.








\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/tarp_approach.pdf}
    \caption{Instantiations of our task-induced representation learning framework. \textbf{Left to right}: Representation learning via multi-task value prediction (\textcolor[HTML]{00A86B}{\textbf{TARP-V}}), via multi-task offline RL (\textcolor[HTML]{F4C430}{\textbf{TARP-CQL}}), via bisimulation (\textcolor[HTML]{796891}{\textbf{TARP-Bisim}}) and via multi-task imitation learning (\textbf{right}, \textcolor[HTML]{FF9090}{\textbf{TARP-BC}}).
    }
    \label{fig:approach}
    \vspace{-1em}
\end{figure}


\section{Task-Induced Representation Learning}
\label{sec:tarp_approach}

An alternative class of representation learning approaches uses task information from prior tasks as a filter for which aspects of the environment are interesting, and which others do not need to be modeled.
This addresses a fundamental problem of unsupervised representation learning approaches: by maximizing the mutual information between observations and representation they are trained to model every bit of information equally and thus can struggle in visually complex environments with lots of irrelevant details.

Formally, the state of an environment $\mathcal{S}$ can be divided into task-relevant and task-irrelevant or nuisance components $\mathcal{S} = \{\mathcal{S}_\text{task}^i, \mathcal{S}_n^i\}$. The superscript $i$ indicates that this division is \emph{task-dependent}, since some components of the state space are relevant for a particular task $T_i$ but irrelevant for others. In visually complex environments, we can assume that $\vert \mathcal{S}_\text{task}\vert \ll \vert \mathcal{S}\vert$, i.e.,~that the task-relevant part of the state space is much smaller than all state information in the input observations~\citep{zhaoping2006theoretical}.

When choosing how much of this input information to model, end-to-end policy learning and unsupervised representation learning, form two ends of a spectrum. End-to-end policy learning only models $\mathcal{S}_\text{task}^i$ for its training task, which is efficient, but only allows transfer from task $i$ to task $j$ if $\mathcal{S}_\text{task}^j \subseteq \mathcal{S}_\text{task}^i$, i.e.,~if the task-relevant components of the target task are a subset of those of the training task. In contrast, unsupervised representation learning models the full $\mathcal{S} = \{\mathcal{S}_\text{task}, \mathcal{S}_n\}$, which allows for flexible transfer since $\mathcal{S}_\text{task}^j \subseteq \mathcal{S} \; \forall\; T_j \in \mathcal{T}$, but training can be inefficient since the learned representation contains many nuisance variables.

In this work, we formalize the family of task-induced representation learning (TARP) approaches, which aim to combine the best of both worlds. Similar to end-to-end policy learning, task-induced representation learning approaches use task information to learn compact, task-relevant representations. Yet, by combining the task information from a wide range of prior tasks they learn a representation that \emph{combines} the task-relevant components of all tasks in the training dataset $\mathcal{D}$: ${\mathcal{S}_\text{TARP} = \mathcal{S}_\text{task}^1 \cup \dots \cup \mathcal{S}_\text{task}^N}$. Thus, such a representation allows for transfer to a wide range of \emph{unseen} tasks %
for which ${\mathcal{S}_\text{task}^\text{target} \subseteq \mathcal{S}_\text{TARP}}$. Yet, the representation filters a large part of the state space which is not relevant for \emph{any} of the training tasks, allowing sample efficient learning on the target task.

\subsection{Approaches for Task-Induced Representation Learning}
\label{sec:tarp_approach_details}

We compare multiple approaches for task-induced representation learning which can leverage different forms of task supervision. We focus on reward annotations and task demonstrations; but, future work can extend the TARP framework to other forms of task supervision like language commands or human preferences. All instantiations of TARP train a shared encoder network $\phi(x)$ with separate task-supervision heads (see Figure~\ref{fig:approach}).

\paragraph{Value Prediction (TARP-V).}
We can leverage reward annotations as task supervision, similar to \citet{fu2021learning}, by estimating the future discounted return of the data collection policy. Intuitively, a representation that allows estimation of the value of a state needs to include all task-relevant aspects of this state. We introduce separate value prediction heads $h_v^i$ for each task $i$ and train the representation $\phi(x)$ by minimizing the error in the predicted discounted return:
\begin{equation}
    \mathcal{L}_\text{TARP-V} = \sum_{i=1}^N \mathbb{E}_{(x_t, r_t) \sim \mathcal{D}_i} \bigg( h_v^i(\phi(x_t)) - \sum_{t^\prime=t}^T \gamma^{t^\prime-t} r_{t^\prime}\bigg)^2.
\end{equation}

\paragraph{Offline RL (TARP-CQL).}
Alternatively, we can learn a representation by training a policy to directly maximize the discounted reward of the training tasks. Since we aim to use offline training data only, we leverage recently proposed methods for offline RL~\citep{levine2020offline,kumar2020conservative} and introduce separate policy heads $h_\pi^i$ and critics $Q^i$ for each task. Following~\citet{kumar2020conservative}, we train the policy to maximize the entropy-augmented future return:
\begin{equation}
    \mathcal{L}_\text{TARP-CQL} = -\sum_{i=1}^N \mathbb{E}_{x \sim \mathcal{D}_i}\bigg(Q^i(x, h_\pi^i(\phi(x))) + \alpha \mathcal{H}\big(h_\pi^i(\phi(x))\big)\bigg).
\end{equation}
Here $\mathcal{H}(\cdot)$ denotes the entropy of the policy's output distribution and $\alpha$ is a learned weighting factor~\citep{kumar2020conservative,haarnoja2018sac_algo_applications}.

\paragraph{Bisimulation (TARP-Bisim).}
We use a bisimulation objective for reward-induced representation learning~\citep{larsen1991bisimulation, ferns2011bisimulation}. It groups states based on their ``behavioral similarity'', measured as their expected future returns under arbitrary action sequences. Specifically, we build on the approach of \citet{zhang2020learning} that leverages deep neural networks to estimate the bisimulation distance, and modify it for multi-task learning by adding per-task embedding heads $z^i = h_\text{bisim}^i\big(\phi(x)\big)$. The representation learning objective is:
\begin{equation}
    \mathcal{L}_\text{TARP-Bisim} = \sum_{i=1}^N \mathbb{E}_{\substack{(x_{j}, a_{j}, r_{j})\\ (x_{k}, a_{k}, r_{k})} \sim \mathcal{D}_i} \bigg( 
    \vert z_j^i - z_k^i \vert - \vert r_j - r_k \vert 
    - \gamma \mathcal{W}_2\big( P(\cdot \vert \bar{z}_{j,t}^i, a_{j,t}), P(\cdot \vert \bar{z}_{k,t}^i, a_{k,t})\big)
    \bigg)^{2} 
\end{equation}
Here $P(\cdot \vert z, a)$ is a learned latent transition model and $\mathcal{W}_2$ refers to the 2-Wasserstein metric which we can compute in closed form for Gaussian transition models. Following \citet{zhang2020learning} we use a target encoder updated with the moving average of the encoder's weights for producing $\bar{z}$ and we add an auxiliary reward prediction objective with per-task reward predictors $\tilde{r}_\text{bisim}^i(z)$. 

\paragraph{Imitation Learning (TARP-BC).}
We can also train task-induced representations from data without reward annotation by directly imitating the data collection policy, thus learning to represent all elements of the state space that were important for the policy's decision making. We choose behavioral cloning (BC,~\citet{pomerleau1989alvinn}) for imitation learning since it is easily applicable especially in the offline setting. We introduce $N$ separate imitation policy heads $h_\text{BC}^i$ and minimize the negative log-likelihood of the training data's actions:
\begin{equation}
    \mathcal{L}_\text{TARP-BC} = - \sum_{i=1}^N \mathbb{E}_{(x, a) \sim \mathcal{D}_i}\bigg(\log h_\text{BC}^i(a \vert \phi(x))\bigg)
\end{equation}





    
    
    
    
    


==> Task-Induced Representation Learning_arXiv/sections/conclusion.tex <==
\section{Conclusion}
In this work, we investigate the effectiveness of representation learning approaches for transfer in visually complex scenes. We define the family of task-induced representation learning approaches, that leverage task-information from prior tasks to only model task-relevant aspects of a scene while ignoring distractors. We compare task-induced representations to common unsupervised representation learning approaches across four visually complex environments with substantial distractors and find that they lead to improved sample efficiency on downstream tasks compared to unsupervised approaches. Future work should investigate approaches for incorporating other sources of task information such as language commands to learn task-induced representation.

==> Task-Induced Representation Learning_arXiv/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}


\subsection{Experimental Setup}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/tarp_envs_w_metaworld.pdf}    
    \caption{Environments with high visual complexity and substantial task-irrelevant detail for testing the learned representations. (a)~\textbf{Distracting DMControl}~\citep{stone2021distracting} with randomly overlayed videos, (b)~\textbf{ViZDoom}~\citep{wydmuch2018vizdoom} with diverse textures and enemy appearances, (c)~\textbf{Distracting MetaWorld}~\citep{yu2019meta} with randomly overlayed videos, and (d)~\textbf{CARLA}~\citep{dosovitskiy17carla} with realistic outdoor driving scenes and weather simulation.
    }
    \label{fig:envs}
    \vspace{-0.5em}
\end{figure}

We compare the performance of different representation learning approaches in four visually complex environments (see Figure~\ref{fig:envs}). We will briefly describe each environment; for more details on environment setup and data collection, see appendix, Section~\ref{sec:environments}.

\paragraph{Distracting DMControl.} We use the environment of~\citet{stone2021distracting}, in which the visual complexity of the standard DMControl ``Walker'' task~\citep{tassa2018deepmind} is increased by overlaying randomly sampled natural videos from the DAVIS~2017 dataset~\citep{pont2017davis}. We train on data collected from standing, forward and backward walking policies and test on a downstream running task. An efficient representation should focus on modeling the agent while ignoring irrelevant information from the background video.

\paragraph{ViZDoom.} A simulator for the ego-shooter game Doom~\citep{wydmuch2018vizdoom}. We use pre-trained models from~\citet{dosovitskiy2016learning} for data collection and vary their objectives to get diverse behaviors such as maximizing the number of collected medi-packs or minimizing the loss of health points. Learned representations should focus on important aspects such as the location of enemies or medi-packs, while ignoring irrelevant details such as the texture of walls or appearance features of medi-packs etc. We test on the full ``battle'' task from \citet{dosovitskiy2016learning}.


\paragraph{Distracting MetaWorld.} Based on the MetaWorld multi-task robotic manipulation environment~\citep{yu2019meta}. We increase the visual complexity by overlaying the background with the same natural videos used in the distracting DMControl, but define a much larger set of 15 training and 6 testing tasks, which require manipulation of diverse objects with a Sawyer robot arm. All objects manipulated in the testing tasks are present in at least one of the training tasks. During evaluation, we report the average performance across the six testing tasks and normalize each task's performance with the score of the best-performing policy. %

\paragraph{Autonomous Driving.} We simulate realistic first-person driving scenarios using the CARLA simulator~\citep{dosovitskiy17carla}.
We collect training data from intersection crossings as well as right and left turns using pre-trained policies and test on a long-range point-to-point driving task that requires navigating an unseen part of the environment. For efficient learning, representations need to model relevant driving information such as position and velocity of other cars, while ignoring irrelevant details such as trees, shadows or the color and make of cars in the scene. 

We compare the different instantiations of the task-induced representation learning framework from Section~\ref{sec:tarp_approach_details} to  common unsupervised representation learning approaches:
\begin{itemize}
    \item \textbf{Reconstruction}: We train a beta-\textbf{VAE}~\citep{higgins2017beta} or a stochastic video prediction model (``\textbf{Pred-O}'') on the training data and transfers the encoder.

    
    
    \item \textbf{Contrastive Learning}: We use the contrastive learning objective from~\citet{stooke2020decoupling} for pre-training (``\textbf{ATC}'').
    
\end{itemize}

We also compare to an approach that combines video prediction with reward prediction for pre-training (``\textbf{Pred-R+O}''), similar to~\citet{hafner2018learning}, thus combining elements form unsupervised and task-induced representation learning. Additionally, we report performance of a \textbf{policy transfer} baseline, which pre-trains a policy on $\mathcal{D}$ using BC and then finetunes the full policy on the downstream task as an alternative to representation transfer\footnote{We also tried pre-training policies on each of the individual task datasets $\mathcal{D}_1, \dots, \mathcal{D}_N$ but found the finetuning performance of the policies trained on the full dataset $\mathcal{D}$ to be superior.}. For environments that provide a low-dimensional state (DMControl, MetaWorld), we further report results for an \textbf{oracle} baseline. %

After pre-training, we transfer the frozen encoder weights to the target task policy, which we train with soft actor-critic (SAC, \citet{haarnoja2018sac}) on continuous control tasks (distracting DMControl, distracting MetaWorld, CARLA), and with PPO~\citep{schulman2017proximal} on discrete action tasks (ViZDoom).\footnote{We report results with finetuning of the pre-trained encoder in appendix, Section~\ref{sec:finetune}, and find no substantial difference to the setting with frozen encoder.}
For more implementation details and hyperparameters, see Appendix~\ref{sec:hyperparams}.


\subsection{Downstream Task Learning Efficiency}
\label{sec:transfer_results_main}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/transfer_performance_w_metaworld.pdf}
    \caption{Performance of transferred representations on unseen target tasks. The task-induced representations (\textcolor[HTML]{0F52BA}{\textbf{blue}}) lead to higher learning efficiency than the fully unsupervised representations or direct policy transfer and achieve comparable performance to the Oracle baseline. All results averaged across three seeds. See Figure~\ref{fig:metaworld_individual_performance} for per-task MetaWorld performances.
    }
    \label{fig:transfer_performance}
    \vspace{-0.5em}
\end{figure}

We report downstream task learning curves for task-induced and unsupervised representation learning methods as well as direct policy transfer in Figure~\ref{fig:transfer_performance}.
The low performance of the \textit{policy transfer} baseline (purple) shows that in most tested environments the downstream task requires significantly different behaviors than those observed in the pre-training data, a scenario in which transferring representations can be beneficial over directly transferring behaviors\footnote{The policy transfer baseline achieves good performance in the distracting DMControl environment since it can reuse behaviors from the \textit{walk-forward} training task for the target \textit{run-forward} task.}.
All reconstruction-based approaches (green) struggle with the complexity of the tested scenes, especially the method that attempts to predict the scene dynamics (\textit{Pred-O}).
We find that adding reward prediction to the objective improves performance (red, \textit{Pred-O+R}). 
Yet, downstream learning is still slow, since the reconstruction objective leads to task-irrelevant information being modeled in the learned representation. The non-reconstructive contrastive approach \textit{ATC} (brown) achieves stronger results, particularly in VizDoom which features less visual distractors, but its performance deteriorates substantially in environments with more task-irrelevant details, i.e. distracted DMControl, MetaWorld and CARLA.


Overall, we find that task-induced representations enable more sample efficient learning. Among the TARP instantiations, we find that TARP-V and TARP-Bisim representations can lead to lower transfer performance, since they rely on the expressiveness of the reward function: if future rewards can be predicted without modeling all task-relevant features, the representations will not capture them. In contrast, TARP-CQL and TARP-BC learn representations via policy learning, which can enable more efficient transfer to downstream policy learning problems. On the distracting DMControl task we find that TARP representations even outperform representations trained with direct supervision through a handcrafted oracle state representation, since they can learn to represent concepts like joint body parts of the walker during pre-training, while the oracle needs to learn these during downstream RL.

\subsection{Probing Task-Induced Representations}

To better understand TARP's improved learning efficiency, we visualize what information is captured in the representation in Figure~\ref{fig:rep_visualization}: we compare input saliency maps for representations learned with task-induced and unsupervised objectives. Saliency maps visualize the average gradient magnitude for each input pixel with respect to the output $\phi(x)$ and thus capture the contribution of each part of the input to the representation. 
We find that task-induced representations focus on the important aspects of the scene, such as the walker agent in distracting DMControl and other cars in CARLA. In contrast, the unsupervised approaches have high saliency values for scattered parts of the input and often represent task-irrelevant aspects such as changing background videos, buildings and trees, since they cannot differentiate task-relevant and irrelevant information.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/rep_visualization.pdf}
    \caption{Visualization of the learned representations. \textbf{Left to right}: saliency maps for representations learned with task-induced representation learning (TARP-BC) and the highest-performing comparisons for reconstruction-based (VAE) and reconstruction-free (ATC) representation learning. \textbf{Left}: Distracting DMControl environment. \textbf{Right}: CARLA environment. Only task-induced representations can ignore distracting information and focus on the important aspects of the scene. 
    }
    \label{fig:rep_visualization}
    \vspace{-0.5em}
\end{figure}

For quantitative analysis, we train probing networks on top of the learned representations in distracting DMControl. We test whether (1)~task-relevant information is modeled by predicting oracle joint states and (2)~whether task-irrelevant information is ignored by classifying the ID of the used background video. The more irrelevant background information is captured in the representation, the better the probing network will be at classifying the video. 
The results show that probing networks trained with task-induced representations more accurately predict the task-relevant state information (Figure~\ref{fig:state_prediction}) while successfully filtering information about the background video and thus obtaining lower background classification accuracy (Figure~\ref{fig:background_classification}). %

\begin{figure}[t]
\begin{minipage}{\textwidth}
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/probing_state_prediction.pdf}
      \caption{State prediction}
      \label{fig:state_prediction}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/probing_background_classification.pdf}
      \caption{Background classification}
      \label{fig:background_classification}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.32\textwidth}
      \includegraphics[width=\linewidth]{figures/IL_performance.pdf}
      \caption{Transfer for imitation learning}
      \label{fig:IL_results}
  \end{subfigure}
   \end{minipage} 
    \caption{(a) Task-induced representations (TARP-BC/V) allow for more accurate prediction of the task-relevant joint states. Unsupervised approaches aim to model all information in the input -- thus probing networks can still learn to predict state information, but struggle to achieve comparably low error rates. (b) Task-induced representations successfully filter task-irrelevant background information and thus cannot confidently classify the background video, while unsupervised approaches fail to filter the irrelevant information and thus achieve perfect classification scores. (c) Transfer performance for IL in distracting DMControl. Task-induced representations achieve superior sample efficiency.
    }
    \label{fig:probing_representation}
    \vspace{-1em}
\end{figure}



    

\subsection{Transferring Representations for Imitation Learning}

We test whether the conclusions from the model-free RL experiments above equally apply when instead performing imitation learning (IL) on the downstream task. We train policies with the pre-trained representations from Section~\ref{sec:transfer_results_main} by Soft-Q Imitation Learning (SQIL, \citet{reddy2020sqil}) on the distracting DMControl target running task.
In Figure~\ref{fig:IL_results} we show that task-induced representations also improve downstream performance in visually complex environments for IL and allow for more efficient imitation, since they model only task-relevant information. Again, TARP-BC and TARP-CQL lead to the best learning efficiency. This shows that the benefit of modeling task-relevant aspects is not constrained to RL, but the \emph{same} representations can be used to accelerate IL.


\subsection{Data Analysis Experiments}
\label{sec:data_analysis}

In the previous sections, we found that task-induced representations can improve learning efficiency over common unsupervised representation learning approaches in visually complex environments. %
These task-induced representation learning approaches are designed to leverage data from a variety of sources, such as prior training runs or human teleoperation. 
Thus, analyzing what characteristics of this training data lead to successful transfer is key to their practical use -- our goal in this section is to derive a set of best practices when collecting datasets for task-induced representation learning.


\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-2.5em}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/metaworld_number_of_tasks_results_w_legend.pdf}    
    \vspace*{-3mm}
    \caption{Transfer performance vs. number of pre-training tasks. Collecting training data from a larger number of tasks is more important for transfer performance than having lots of data for few tasks.
    }
    \label{fig:number_of_tasks}
    \vspace{-2em}
\end{wrapfigure}

\paragraph{Many tasks vs. lots of data per task.} When collecting large datasets there is a trade-off between collecting a lot of data for few tasks vs. collecting less data each for a larger set of tasks. To analyze the effects of this trade-off on TARP, we train TARP-BC on data from a varying number of pre-training tasks in distracting MetaWorld. When training on data from fewer tasks, we collect more data on each of these tasks, to ensure that the size of the training datasets is constant across all experiments.
The results in Figure~\ref{fig:number_of_tasks} show: \textbf{training on fewer data from a larger number of tasks is beneficial over training on lots of data from few tasks}.
Intuitively, since downstream tasks can leverage the union of task-relevant components of all training tasks, having a diverse set of tasks is more important for transfer than having lots of data for few tasks.


\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/data_analysis_results.pdf}
    \vspace*{-3mm}
    \caption{Robustness to pre-training data optimality. TARP approaches can learn good representations that allow for effective transfer even from sub-optimal data.
    }
    \label{fig:data_quality}
    \vspace{-1em}
\end{wrapfigure}

\paragraph{More data vs. optimal data.} Another trade-off in data collection exists between the amount of data and its optimality: a method that can learn from sub-optimal trajectory data is able to leverage much larger and more diverse datasets. Since training on diverse data is important for successful transfer (see above) robustness to sub-optimal training data is an important feature of any representation learning approach. We test the robustness of task-induced representation learning approaches by training on sub-optimal trajectory data, collected from only partially trained and completely random policies, in distracting DMControl. The downstream RL performance comparison in Figure~\ref{fig:data_quality} shows that TARP approaches can learn strong representations from low-performance trajectory data and even when trained from random data, performance does not decrease compared to a SAC baseline trained from scratch. Intuitively, task-induced representation learning does not pre-train a model on ``how to act'' but merely ``what to pay attention to''. We find that TARP-CQL's performance can even increase slightly with the suboptimal data, which we attribute to its increased state coverage.
Thus we conclude that task-induced representation learning is robust to the optimality of the pre-training data and \textbf{collecting larger, diverse datasets is more important than collecting optimal data}.


\paragraph{Multi-Source Task Supervision.}
When collecting large datasets, it can be beneficial to pool data from multiple sources, e.g. data obtained from prior training runs or via human teleoperation. In Section~\ref{sec:tarp_approach} we introduced different instantiations of the TARP framework that are able to leverage different forms of task supervision. Here, we test whether we can train a single representation using multiple sources of task supervision simultaneously. In particular, we train ``TARP-V+BC'' models that assume reward annotations for only some of the tasks in the pre-training dataset and demonstration data for the remaining tasks (for more details on data collection, see Section~\ref{sec:multi_source}).
We compare downstream learning efficiency on distracting DMControl and CARLA in Figure~\ref{fig:single_vs_multi}
We find that the combined-source model trained from the heterogeneous dataset achieves comparable or superior performance to all single-source models, showing that practitioners should \textbf{collect diverse datasets, even if they have heterogeneous sources of task-supervision}. 




    



    
    





==> Task-Induced Representation Learning_arXiv/sections/introduction.tex <==
\section{Introduction}


The ability to compress sensory inputs into a compact representation is crucial for effective decision making. Deep reinforcement learning (RL) has enabled the learning of such representations via end-to-end policy training~\citep{mnih_nature_2015,levine2016end}. However, learning representations from reward feedback requires many environment interactions. Instead, \emph{unsupervised} objectives for representation learning~\citep{lange2010deep,finn2016deep,hafner2018learning,oord2018representation,chen2020simclr} directly maximize lower bounds on the mutual information between the sensory inputs and the learned representation. Empirically, such unsupervised objectives can accelerate the training of deep RL agents substantially~\citep{laskin2020curl,stooke2020decoupling,yang2021representation}. However, prior works have evaluated such representation learning approaches in clean laboratory or simulated settings~\citep{finn2016deep,lee2019stochastic,laskin2020curl} where most of the perceived information is important for the task at hand. In contrast, realistic environments feature lots of task-irrelevant detail, such as clutter or objects moving in the background. This has the potential to impair the performance of unsupervised representations for RL since they aim to model \emph{all} information in the input equally.

The goal of this paper is to evaluate the effectiveness of representation learning approaches for decision making in such more realistic, visually complex environments with distractors and clutter. We evaluate two classes of representation learning approaches: (1)~unsupervised representation learning based on reconstruction, prediction or contrastive objectives, and (2)~approaches that leverage task information from prior tasks to shape the representation, which we will refer to as \emph{task-induced representation learning} approaches. Such task information can often be available at no extra cost, \eg in the form of prior task rewards if the data has been collected from RL training runs. Task-induced representations can leverage this task information to determine which features are important in visually complex scenes, and which are distractors that can be ignored. 
We focus our evaluation on a practical representation learning setting, shown in Figure~\ref{fig:teaser}: given a large offline dataset of experience collected across multiple prior tasks, we perform offline representation learning with different approaches. Then, we transfer the pre-trained representations for training a policy on a new task and compare efficiency to training the policy from scratch. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/tarp_teaser.pdf}
    \caption{Overview of our pipeline for evaluating representation learning in visually complex scenes: given a multi-task dataset of prior experience we pre-train representations using unsupervised objectives, such as prediction and contrastive learning, or task-induced approaches, which leverage task-information from prior tasks to learn to focus on task-relevant aspects of the scene. We then evaluate the efficiency of the pre-trained representations for learning unseen tasks.
    }
    \label{fig:teaser}
    \vspace{-1.2em}
\end{figure}


To evaluate the effectiveness of different representation learning objectives, we compare common unsupervised approaches based on reconstruction, prediction and contrastive learning to four task-induced representation learning methods. We perform experiments in four visually complex environments, ranging from scenes with distracting background videos in the Distracting DMControl bench~\citep{stone2021distracting} to realistic distractors such as clouds, weather and urban scenery in the CARLA driving simulator~\citep{dosovitskiy17carla}. Across RL and imitation learning experiments we find that pre-trained representations accelerate downstream task learning, even in visually complex environments. Additionally, in our comparisons task-induced representation learning approaches achieve up to double the learning efficiency of unsupervised approaches by learning to ignore distractors and task-irrelevant visual details.

In summary, the contributions of our work are threefold: (1)~we formalize the class of \emph{task-induced representation learning} approaches which leverage task-information from prior tasks for shaping the learned representations, (2)~we empirically compare widely used unsupervised representation learning approaches and task-induced representation learning methods across four visually complex environments with numerous distractors, showing that task-induced representations can lead to more effective learning and (3)~through analysis experiments we develop a set of best practices for task-induced representation learning.


















==> Task-Induced Representation Learning_arXiv/sections/related_work.tex <==
    \section{Related Work}
\label{sec:related_work}

    
    




Deep RL %
can train \textbf{``end-to-end'' policies} that directly map raw visual inputs to action commands~\citep{mnih_nature_2015,kalashnikov2018scalable}. 
To improve data efficiency in deep RL from high-dimensional observations, a number of recent works %
have explored using data augmentation~\citep{kostrikov2020image,laskin2020reinforcement} and \textbf{unsupervised representation learning} techniques during RL training. The latter can be categorized into (1)~reconstruction~\citep{lange2010deep,finn2016deep}, (2)~prediction~\citep{hafner2018learning,lee2019stochastic}, and (3)~contrastive learning~\citep{laskin2020curl,stooke2020decoupling,zhan2020framework,yang2021representation} approaches. While these works have shown improved sample efficiency, fundamentally they are \emph{unsupervised} and therefore cannot decide which information in the input is relevant or irrelevant to a certain task. We show that this leads to deteriorating performance in visually complex environments such as autonomous driving scenarios with lots of non-relevant information in the input observations. 

Another line of work has used task information to shape representations that learn to ignore distractors. Specifically, \citet{fu2021learning} predict future rewards to learn representations that focus only on task-relevant aspects of a scene. \citet{zhang2020learning} leverage rewards as part of a bisimulation objective to learn representations without reconstruction. In this work, we provide a unifying framework for such task-induced representation learning approaches that encompasses the objectives of \citet{fu2021learning} and \citet{zhang2020learning} among others, and perform a systematic comparison to unsupervised representations in visually complex environments.

Closest to our work is the work of \citet{yang2021representation}, which evaluates unsupervised and task-induced representation learning objectives for pre-training in multiple environments from the D4RL benchmark~\citep{fu2020d4rl}. Their work shows that representation pre-training can substantially improve downstream learning efficiency. While \citet{yang2021representation}'s evaluation is performed in visually clean OpenAI gym environments~\citep{brockman2016openai} without distractors, we focus our evaluation on more realistic, visually complex environments with distractors, which can pose additional challenges, especially for unsupervised representation learning approaches.





==> Task-Induced Representation Learning_arXiv/sections/reproducibility.tex <==
\section{Reproducibility Statement}
We provide a detailed description of all used environments, the procedures for offline dataset collection, and descriptions of the downstream evaluation tasks in appendix, Section~\ref{sec:environments}. Furthermore, in appendix, Section~\ref{sec:hyperparams} we list all hyperparameters used for the pre-training phase (i.e. task-induced and unsupervised representation learning) as well as for training of the RL policies. We open-source our codebase with example commands to reproduce our results on the project website: \href{https://clvrai.com/tarp}{\url{clvrai.com/tarp}}.

